Lifted Tree-Reweighted Variational Inference

We analyze variational inference for highly symmetric graphical models such as those arising from first-order probabilistic models. We first show that for these graphical models, the tree-reweighted variational objective lends itself to a compact lifted formulation which can be solved much more efficiently than the standard TRW formulation for the ground graphical model. Compared to earlier work on lifted belief propagation, our formulation leads to a convex optimization problem for lifted marginal inference and provides an upper bound on the partition function. We provide two approaches for improving the lifted TRW upper bound. The first is a method for efficiently computing maximum spanning trees in highly symmetric graphs, which can be used to optimize the TRW edge appearance probabilities. The second is a method for tightening the relaxation of the marginal polytope using lifted cycle inequalities and novel exchangeable cluster consistency constraints.

==> algorithm_template.tex <==
\begin{algorithm}
\caption{Sample algorithm\\
Find~$\max_{q}P(q)=\frac{1}{Z}F(q)\prod_{i=1}^{n}\phi_{i}(q_{i})$\\
Input:~$c_{k}=F(q)$;~$\alpha_{i}=\frac{\phi_{i}(1)}{\phi_{i}(0)}$
}
\label{alg:map}
\begin{algorithmic}[1]
\State $(\alpha', order) \gets  sort(\alpha_{1},\ldots,\alpha_{n})$~in~descending~order
\State $prod\alpha' \gets 1$; $maxval \gets c_0$; $k \gets 0$
\For{i=1,\dots,n}
\State $prod\alpha' \gets prod\alpha' \times \alpha'_i$
\If{$c_i \times prod\alpha' > maxval$}
	\State $maxval \gets c_i \times prod\alpha'$
	\State $k = i$
\EndIf
\EndFor
\State \textbf{return} $q$ where\\
$q_{i}=\begin{cases}
1 & \text{{\,\ if\,\mbox{\ensuremath{order(i)\leq k}}}}\\
0 & \text{{\,\ otherwise}}
\end{cases}$
\end{algorithmic}
\end{algorithm}


==> cliqueCycleMLN.tex <==
\begin{eqnarray*}
w & x \neq y \wedge Q1(x) \wedge Q2(y)\\
w & x \neq y \wedge Q2(x) \wedge Q3(y)\\
w & x \neq y \wedge Q3(x) \wedge Q1(y)\\

-w & x \neq y \wedge Q1(x) \wedge Q1(y)\\
-w & x \neq y \wedge Q2(x) \wedge Q2(y)\\
-w & x \neq y \wedge Q3(x) \wedge Q3(y)\\
\end{eqnarray*}
